The Association of Opening K-12 Schools with the Spread of COVID-19 in the United States: County-Level Panel Data Analysis

This paper empirically examines how the opening of K-12 schools and colleges is associated with the spread of COVID-19 using county-level panel data in the United States. Using data on foot traffic and K-12 school opening plans, we analyze how an increase in visits to schools and opening schools with different teaching methods (in-person, hybrid, and remote) is related to the 2-weeks forward growth rate of confirmed COVID-19 cases. Our debiased panel data regression analysis with a set of county dummies, interactions of state and week dummies, and other controls shows that an increase in visits to both K-12 schools and colleges is associated with a subsequent increase in case growth rates. The estimates indicate that fully opening K-12 schools with in-person learning is associated with a 5 (SE = 2) percentage points increase in the growth rate of cases. We also find that the positive association of K-12 school visits or in-person school openings with case growth is stronger for counties that do not require staff to wear masks at schools. These results have a causal interpretation in a structural model with unobserved county and time confounders. Sensitivity analysis shows that the baseline results are robust to timing assumptions and alternative specifications.

==> tables_and_figures/behavior-fulltime-fe-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & Full-time Workplace Visits & Full-time Workplace Visits & Staying Home Devices & Staying Home Devices \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Mandatory mask & $-$0.057 & $-$0.141$^{**}$ & 0.016 & 0.036 \\ 
  & (0.042) & (0.053) & (0.259) & (0.250) \\ 
  Ban gatherings & 0.060 & 0.075 & 0.436 & 0.351 \\ 
  & (0.047) & (0.051) & (0.560) & (0.520) \\ 
  Stay at Staying Home Devices & $-$0.060$^{*}$ & $-$0.066$^{*}$ & 2.793$^{***}$ & 2.809$^{***}$ \\ 
  & (0.031) & (0.033) & (0.329) & (0.340) \\ 
  College Visits & $-$0.040$^{***}$ & $-$0.046$^{***}$ & $-$0.144$^{***}$ & $-$0.148$^{***}$ \\ 
  & (0.004) & (0.006) & (0.024) & (0.026) \\ 
  K-12 School Visits & 0.085$^{***}$ &  & $-$0.019 &  \\ 
  & (0.006) &  & (0.026) &  \\ 
  Open K-12 In-person &  & 0.999$^{***}$ &  & $-$0.924$^{**}$ \\ 
  &  & (0.125) &  & (0.382) \\ 
  Open K-12 Hybrid &  & 0.490$^{***}$ &  & $-$0.127 \\ 
  &  & (0.051) &  & (0.186) \\ 
  Open K-12 Remote &  & 0.236$^{***}$ &  & $-$0.271 \\ 
  &  & (0.048) &  & (0.307) \\ 
  log(Cases) & 0.005 & 0.003 & 0.288$^{***}$ & 0.282$^{***}$ \\ 
  & (0.004) & (0.005) & (0.028) & (0.028) \\ 
  lag(log(Cases), 7) & $-$0.001 & $-$0.005$^{*}$ & 0.209$^{***}$ & 0.207$^{***}$ \\ 
  & (0.002) & (0.003) & (0.019) & (0.017) \\ 
  lag(log(Cases), 14) & $-$0.0005 & $-$0.003 & 0.098$^{***}$ & 0.097$^{***}$ \\ 
  & (0.002) & (0.002) & (0.023) & (0.024) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 670,895 & 595,872 & 670,895 & 595,872 \\ 
R$^{2}$ & 0.870 & 0.853 & 0.889 & 0.888 \\ 
Adjusted R$^{2}$ & 0.869 & 0.851 & 0.888 & 0.887 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-fulltime-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & fullwork & fullwork & home & home \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Mandatory mask & $-$0.152$^{***}$ & $-$0.306$^{***}$ & 0.204 & 0.222 \\ 
  & (0.042) & (0.053) & (0.260) & (0.250) \\ 
  Ban gatherings & 0.067 & 0.097$^{*}$ & 0.870 & 0.754 \\ 
  & (0.047) & (0.051) & (0.561) & (0.521) \\ 
  Stay at home & $-$0.039 & $-$0.028 & 2.881$^{***}$ & 2.895$^{***}$ \\ 
  & (0.031) & (0.033) & (0.330) & (0.340) \\ 
  College Visits & $-$0.080$^{***}$ & $-$0.098$^{***}$ & $-$0.207$^{***}$ & $-$0.207$^{***}$ \\ 
  & (0.004) & (0.006) & (0.024) & (0.026) \\ 
  K-12 Visits & 0.078$^{***}$ &  & $-$0.061$^{**}$ &  \\ 
  & (0.006) &  & (0.026) &  \\ 
  Open K-12 In-person &  & 0.999$^{***}$ &  & $-$2.271$^{***}$ \\ 
  &  & (0.125) &  & (0.382) \\ 
  Open K-12 Hybrid &  & 0.509$^{***}$ &  & 0.094 \\ 
  &  & (0.051) &  & (0.186) \\ 
  Open K-12 Remote &  & 0.211$^{***}$ &  & 0.159 \\ 
  &  & (0.048) &  & (0.307) \\ 
  log(Cases), 14d lag & 0.004 & 0.007 & 0.273$^{***}$ & 0.273$^{***}$ \\ 
  & (0.004) & (0.005) & (0.028) & (0.028) \\ 
  lag(log(Cases), 14d lag, 7) & 0.002 & $-$0.001 & 0.283$^{***}$ & 0.281$^{***}$ \\ 
  & (0.002) & (0.003) & (0.019) & (0.017) \\ 
  lag(log(Cases), 14d lag, 14) & 0.006$^{***}$ & 0.005$^{*}$ & 0.221$^{***}$ & 0.215$^{***}$ \\ 
  & (0.002) & (0.002) & (0.023) & (0.024) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 670,909 & 595,886 & 670,909 & 595,886 \\ 
R$^{2}$ & 0.870 & 0.853 & 0.889 & 0.888 \\ 
Adjusted R$^{2}$ & 0.869 & 0.851 & 0.888 & 0.887 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-restaurant-fe-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & Restaurant Visits & Restaurant Visits & Bar Visits & Bar Visits \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Mandatory mask & 1.096$^{***}$ & 0.744$^{*}$ & 0.180$^{***}$ & 0.116 \\ 
  & (0.371) & (0.403) & (0.067) & (0.069) \\ 
  Ban gatherings & $-$0.545 & $-$0.477 & $-$0.103 & $-$0.105 \\ 
  & (0.920) & (0.897) & (0.117) & (0.118) \\ 
  Stay at Staying Home Devices & $-$1.885$^{***}$ & $-$1.870$^{***}$ & $-$0.182$^{***}$ & $-$0.167$^{***}$ \\ 
  & (0.203) & (0.242) & (0.025) & (0.025) \\ 
  College Visits & 0.288$^{***}$ & 0.270$^{***}$ & 0.022$^{***}$ & 0.020$^{***}$ \\ 
  & (0.053) & (0.051) & (0.006) & (0.005) \\ 
  K-12 School Visits & 0.094$^{**}$ &  & 0.012$^{**}$ &  \\ 
  & (0.046) &  & (0.006) &  \\ 
  Open K-12 In-person &  & $-$0.578 &  & $-$0.059 \\ 
  &  & (0.404) &  & (0.041) \\ 
  Open K-12 Hybrid &  & $-$0.991$^{***}$ &  & $-$0.101$^{***}$ \\ 
  &  & (0.272) &  & (0.038) \\ 
  Open K-12 Remote &  & $-$0.785$^{**}$ &  & $-$0.006 \\ 
  &  & (0.295) &  & (0.056) \\ 
  log(Cases) & $-$0.020 & $-$0.019 & $-$0.001 & 0.002 \\ 
  & (0.047) & (0.050) & (0.006) & (0.007) \\ 
  lag(log(Cases), 7) & $-$0.026 & $-$0.039 & $-$0.005 & $-$0.003 \\ 
  & (0.032) & (0.032) & (0.005) & (0.005) \\ 
  lag(log(Cases), 14) & $-$0.066 & $-$0.078$^{*}$ & $-$0.007 & $-$0.009 \\ 
  & (0.043) & (0.042) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 670,895 & 595,872 & 670,895 & 595,872 \\ 
R$^{2}$ & 0.881 & 0.883 & 0.807 & 0.807 \\ 
Adjusted R$^{2}$ & 0.880 & 0.882 & 0.806 & 0.806 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/behavior-restaurant-pib.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & Restaurant Visits & Restaurant Visits & Bar Visits & Bar Visits \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Mandatory mask & 0.542 & 0.037 & 0.191$^{***}$ & 0.113 \\ 
  & (0.371) & (0.403) & (0.067) & (0.069) \\ 
  Ban gatherings & 0.067 & 0.135 & $-$0.066 & $-$0.070 \\ 
  & (0.920) & (0.897) & (0.117) & (0.118) \\ 
  Stay at home & $-$2.232$^{***}$ & $-$2.170$^{***}$ & $-$0.228$^{***}$ & $-$0.204$^{***}$ \\ 
  & (0.203) & (0.241) & (0.025) & (0.025) \\ 
  College Visits & 0.064 & 0.034 & 0.016$^{***}$ & 0.012$^{**}$ \\ 
  & (0.053) & (0.051) & (0.006) & (0.005) \\ 
  K-12 Visits & 0.006 &  & 0.008 &  \\ 
  & (0.046) &  & (0.006) &  \\ 
  Open K-12 In-person &  & $-$1.367$^{***}$ &  & $-$0.177$^{***}$ \\ 
  &  & (0.404) &  & (0.041) \\ 
  Open K-12 Hybrid &  & $-$1.162$^{***}$ &  & $-$0.097$^{***}$ \\ 
  &  & (0.272) &  & (0.038) \\ 
  Open K-12 Remote &  & $-$0.512$^{*}$ &  & 0.031 \\ 
  &  & (0.295) &  & (0.056) \\ 
  log(Cases), 14d lag & $-$0.096$^{**}$ & $-$0.072 & $-$0.010$^{*}$ & $-$0.004 \\ 
  & (0.047) & (0.050) & (0.006) & (0.007) \\ 
  lag(log(Cases), 14d lag, 7) & $-$0.084$^{***}$ & $-$0.087$^{***}$ & $-$0.011$^{**}$ & $-$0.009$^{*}$ \\ 
  & (0.032) & (0.032) & (0.005) & (0.005) \\ 
  lag(log(Cases), 14d lag, 14) & $-$0.150$^{***}$ & $-$0.161$^{***}$ & $-$0.014$^{**}$ & $-$0.015$^{***}$ \\ 
  & (0.043) & (0.042) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 670,909 & 595,886 & 670,909 & 595,886 \\ 
R$^{2}$ & 0.881 & 0.883 & 0.807 & 0.807 \\ 
Adjusted R$^{2}$ & 0.880 & 0.882 & 0.806 & 0.806 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.055$^{**}$ & $-$0.054$^{**}$ & $-$0.058$^{**}$ & $-$0.063$^{**}$ \\ 
  & (0.025) & (0.026) & (0.026) & (0.027) \\ 
  lag(Ban gatherings, 14) & $-$0.052 & $-$0.054 & $-$0.064 & $-$0.052 \\ 
  & (0.044) & (0.056) & (0.042) & (0.053) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.144$^{***}$ & $-$0.128$^{***}$ & $-$0.139$^{***}$ & $-$0.136$^{***}$ \\ 
  & (0.038) & (0.044) & (0.040) & (0.044) \\ 
  lag(College Visits, 14) & 0.042 & 0.022 & $-$0.027 & 0.001 \\ 
  & (0.069) & (0.069) & (0.072) & (0.072) \\ 
  lag(K-12 School Visits, 14) & 0.328$^{*}$ & 0.335 &  &  \\ 
  & (0.183) & (0.200) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.128 &  &  \\ 
  &  & (0.082) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.007 & 0.004 \\ 
  &  &  & (0.018) & (0.023) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.001 & $-$0.004 \\ 
  &  &  & (0.014) & (0.015) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.007 & 0.003 \\ 
  &  &  & (0.019) & (0.018) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & $-$0.008 \\ 
  &  &  &  & (0.019) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.006 \\ 
  &  &  &  & (0.018) \\ 
  lag(Test Growth Rates, 14) & $-$0.0003 & $-$0.002 & $-$0.0004 & $-$0.001 \\ 
  & (0.002) & (0.002) & (0.002) & (0.002) \\ 
  Test Growth Rates & 0.007 & 0.006 & 0.007 & 0.007 \\ 
  & (0.005) & (0.005) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 763,154 & 603,514 & 677,828 & 585,593 \\ 
R$^{2}$ & 0.074 & 0.075 & 0.074 & 0.075 \\ 
Adjusted R$^{2}$ & 0.068 & 0.067 & 0.067 & 0.068 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.278$^{***}$ & $-$0.244$^{***}$ & $-$0.270$^{***}$ & $-$0.256$^{***}$ \\ 
  & (0.048) & (0.051) & (0.050) & (0.052) \\ 
  lag(Ban gatherings, 14) & $-$0.112 & $-$0.067 & $-$0.113 & $-$0.055 \\ 
  & (0.155) & (0.151) & (0.155) & (0.149) \\ 
  lag(Stay at Staying Home Devices, 14) & 0.412$^{***}$ & 0.435$^{***}$ & 0.464$^{***}$ & 0.469$^{***}$ \\ 
  & (0.066) & (0.073) & (0.071) & (0.079) \\ 
  lag(College Visits, 14) & 1.927$^{***}$ & 2.016$^{***}$ & 1.945$^{***}$ & 1.879$^{***}$ \\ 
  & (0.253) & (0.264) & (0.233) & (0.254) \\ 
  lag(K-12 School Visits, 14) & 1.402$^{***}$ & 0.978$^{***}$ &  &  \\ 
  & (0.193) & (0.222) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.792$^{***}$ &  &  \\ 
  &  & (0.194) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.338$^{***}$ & 0.303$^{***}$ \\ 
  &  &  & (0.046) & (0.048) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.150$^{***}$ & 0.104$^{***}$ \\ 
  &  &  & (0.029) & (0.031) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.013 & 0.009 \\ 
  &  &  & (0.038) & (0.044) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.059 \\ 
  &  &  &  & (0.057) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.167$^{***}$ \\ 
  &  &  &  & (0.048) \\ 
  lag(log(Cases), 14) & 0.408$^{***}$ & 0.405$^{***}$ & 0.409$^{***}$ & 0.402$^{***}$ \\ 
  & (0.010) & (0.009) & (0.010) & (0.009) \\ 
  lag(lag(log(Cases), 7), 14) & 0.133$^{***}$ & 0.135$^{***}$ & 0.133$^{***}$ & 0.134$^{***}$ \\ 
  & (0.005) & (0.004) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & 0.025$^{***}$ & 0.027$^{***}$ & 0.023$^{***}$ & 0.025$^{***}$ \\ 
  & (0.006) & (0.005) & (0.006) & (0.006) \\ 
  Test Growth Rates & 0.005$^{**}$ & 0.004$^{*}$ & 0.005$^{**}$ & 0.004$^{*}$ \\ 
  & (0.002) & (0.002) & (0.002) & (0.002) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 760,422 & 600,958 & 675,405 & 583,119 \\ 
R$^{2}$ & 0.867 & 0.862 & 0.866 & 0.861 \\ 
Adjusted R$^{2}$ & 0.866 & 0.861 & 0.865 & 0.859 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt0-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d2log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.519$^{***}$ & $-$0.536$^{***}$ & $-$0.507$^{***}$ & $-$0.512$^{***}$ \\ 
  & (0.043) & (0.041) & (0.043) & (0.041) \\ 
  lag(Ban gatherings, 14) & $-$0.403$^{***}$ & $-$0.405$^{***}$ & $-$0.427$^{***}$ & $-$0.415$^{***}$ \\ 
  & (0.046) & (0.069) & (0.055) & (0.070) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.294$^{***}$ & $-$0.273$^{**}$ & $-$0.269$^{***}$ & $-$0.262$^{**}$ \\ 
  & (0.095) & (0.114) & (0.104) & (0.123) \\ 
  lag(College Visits, 14) & 0.226 & $-$0.346 & 0.205 & $-$0.328 \\ 
  & (0.240) & (0.260) & (0.230) & (0.252) \\ 
  lag(K-12 School Visits, 14) & 1.185$^{***}$ & 0.469$^{***}$ &  &  \\ 
  & (0.142) & (0.155) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 1.324$^{***}$ &  &  \\ 
  &  & (0.176) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.241$^{***}$ & 0.115$^{***}$ \\ 
  &  &  & (0.041) & (0.041) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & $-$0.023 & $-$0.139$^{***}$ \\ 
  &  &  & (0.028) & (0.029) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.337$^{***}$ & $-$0.369$^{***}$ \\ 
  &  &  & (0.028) & (0.032) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.115$^{*}$ \\ 
  &  &  &  & (0.059) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.174$^{***}$ \\ 
  &  &  &  & (0.040) \\ 
  lag(log(Cases), 14) & $-$0.231$^{***}$ & $-$0.220$^{***}$ & $-$0.220$^{***}$ & $-$0.212$^{***}$ \\ 
  & (0.012) & (0.010) & (0.012) & (0.010) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.457$^{***}$ & $-$0.456$^{***}$ & $-$0.453$^{***}$ & $-$0.453$^{***}$ \\ 
  & (0.007) & (0.007) & (0.007) & (0.007) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.009 & $-$0.005 & $-$0.004 & $-$0.003 \\ 
  & (0.006) & (0.006) & (0.006) & (0.006) \\ 
  Test Growth Rates & 0.001 & 0.0005 & 0.001 & 0.001 \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 668,101 & 527,576 & 593,265 & 511,939 \\ 
R$^{2}$ & 0.375 & 0.376 & 0.372 & 0.377 \\ 
Adjusted R$^{2}$ & 0.370 & 0.371 & 0.367 & 0.372 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt1-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.028 & 0.013 & $-$0.027 & $-$0.006 \\ 
  & (0.041) & (0.039) & (0.044) & (0.042) \\ 
  lag(Ban gatherings, 14) & $-$0.363$^{***}$ & $-$0.323$^{***}$ & $-$0.360$^{***}$ & $-$0.317$^{***}$ \\ 
  & (0.098) & (0.082) & (0.097) & (0.080) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.151$^{**}$ & $-$0.128$^{*}$ & $-$0.155$^{**}$ & $-$0.130$^{*}$ \\ 
  & (0.060) & (0.068) & (0.064) & (0.073) \\ 
  lag(College Visits, 14) & 1.444$^{***}$ & 1.778$^{***}$ & 1.442$^{***}$ & 1.584$^{***}$ \\ 
  & (0.202) & (0.204) & (0.179) & (0.197) \\ 
  lag(K-12 School Visits, 14) & 1.345$^{***}$ & 1.155$^{***}$ &  &  \\ 
  & (0.142) & (0.139) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.246 &  &  \\ 
  &  & (0.159) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.390$^{***}$ & 0.360$^{***}$ \\ 
  &  &  & (0.041) & (0.040) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.268$^{***}$ & 0.240$^{***}$ \\ 
  &  &  & (0.025) & (0.025) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.192$^{***}$ & 0.213$^{***}$ \\ 
  &  &  & (0.027) & (0.031) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.037 \\ 
  &  &  &  & (0.050) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.131$^{***}$ \\ 
  &  &  &  & (0.037) \\ 
  lag(log(Cases)\_F7, 14) & 0.518$^{***}$ & 0.511$^{***}$ & 0.516$^{***}$ & 0.509$^{***}$ \\ 
  & (0.015) & (0.014) & (0.016) & (0.014) \\ 
  lag(log(Cases), 14) & 0.240$^{***}$ & 0.232$^{***}$ & 0.237$^{***}$ & 0.229$^{***}$ \\ 
  & (0.008) & (0.009) & (0.009) & (0.009) \\ 
  lag(lag(log(Cases), 7), 14) & 0.061$^{***}$ & 0.062$^{***}$ & 0.061$^{***}$ & 0.061$^{***}$ \\ 
  & (0.005) & (0.004) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & 0.015$^{***}$ & 0.015$^{***}$ & 0.014$^{***}$ & 0.013$^{***}$ \\ 
  & (0.004) & (0.004) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{***}$ & 0.008$^{**}$ & 0.009$^{***}$ & 0.008$^{**}$ \\ 
  & (0.003) & (0.003) & (0.003) & (0.003) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 677,420 & 535,085 & 601,553 & 519,205 \\ 
R$^{2}$ & 0.876 & 0.871 & 0.875 & 0.870 \\ 
Adjusted R$^{2}$ & 0.875 & 0.870 & 0.874 & 0.869 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt2-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d2log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.117$^{**}$ & $-$0.118$^{**}$ & $-$0.129$^{**}$ & $-$0.137$^{**}$ \\ 
  & (0.046) & (0.052) & (0.051) & (0.055) \\ 
  lag(Ban gatherings, 14) & $-$0.199$^{***}$ & $-$0.209$^{**}$ & $-$0.205$^{***}$ & $-$0.214$^{**}$ \\ 
  & (0.065) & (0.090) & (0.066) & (0.094) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.293$^{***}$ & $-$0.266$^{***}$ & $-$0.285$^{***}$ & $-$0.254$^{***}$ \\ 
  & (0.038) & (0.034) & (0.039) & (0.035) \\ 
  lag(College Visits, 14) & 0.524$^{***}$ & 0.481$^{**}$ & 0.444$^{***}$ & 0.434$^{**}$ \\ 
  & (0.154) & (0.181) & (0.158) & (0.177) \\ 
  lag(K-12 School Visits, 14) & 0.819$^{***}$ & 0.837$^{***}$ &  &  \\ 
  & (0.157) & (0.149) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.110 &  &  \\ 
  &  & (0.120) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.051$^{*}$ & 0.044 \\ 
  &  &  & (0.030) & (0.035) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.027$^{*}$ & 0.015 \\ 
  &  &  & (0.016) & (0.019) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.012 & $-$0.005 \\ 
  &  &  & (0.024) & (0.025) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & $-$0.002 \\ 
  &  &  &  & (0.033) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & $-$0.002 \\ 
  &  &  &  & (0.031) \\ 
  lag(const, 14) &  &  &  &  \\ 
  &  &  &  &  \\ 
  Test Growth Rates & 0.002 & 0.001 & 0.002 & 0.001 \\ 
  & (0.002) & (0.002) & (0.002) & (0.002) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 754,765 & 596,796 & 670,375 & 579,094 \\ 
R$^{2}$ & 0.165 & 0.160 & 0.161 & 0.160 \\ 
Adjusted R$^{2}$ & 0.159 & 0.154 & 0.155 & 0.154 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt2-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d2log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.104$^{**}$ & $-$0.092$^{*}$ & $-$0.107$^{**}$ & $-$0.113$^{**}$ \\ 
  & (0.046) & (0.052) & (0.051) & (0.055) \\ 
  lag(Ban gatherings, 14) & $-$0.230$^{***}$ & $-$0.214$^{**}$ & $-$0.213$^{***}$ & $-$0.204$^{**}$ \\ 
  & (0.065) & (0.090) & (0.066) & (0.094) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.309$^{***}$ & $-$0.263$^{***}$ & $-$0.275$^{***}$ & $-$0.245$^{***}$ \\ 
  & (0.038) & (0.034) & (0.039) & (0.035) \\ 
  lag(College Visits, 14) & 0.309$^{**}$ & 0.195 & 0.100 & 0.028 \\ 
  & (0.154) & (0.181) & (0.158) & (0.177) \\ 
  lag(K-12 School Visits, 14) & 0.732$^{***}$ & 0.653$^{***}$ &  &  \\ 
  & (0.157) & (0.149) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.339$^{***}$ &  &  \\ 
  &  & (0.120) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.104$^{***}$ & 0.149$^{***}$ \\ 
  &  &  & (0.030) & (0.035) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.037$^{**}$ & 0.014 \\ 
  &  &  & (0.016) & (0.019) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.028 & $-$0.008 \\ 
  &  &  & (0.024) & (0.025) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & $-$0.072$^{**}$ \\ 
  &  &  &  & (0.033) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.038 \\ 
  &  &  &  & (0.031) \\ 
  lag(const, 14) &  &  &  &  \\ 
  &  &  &  &  \\ 
  Test Growth Rates & 0.002 & 0.001 & 0.002 & 0.001 \\ 
  & (0.002) & (0.002) & (0.002) & (0.002) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 754,765 & 596,796 & 670,375 & 579,094 \\ 
R$^{2}$ & 0.165 & 0.160 & 0.161 & 0.160 \\ 
Adjusted R$^{2}$ & 0.159 & 0.154 & 0.155 & 0.154 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt3-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d2log(Cases)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 21) & $-$0.112$^{***}$ & $-$0.107$^{**}$ & $-$0.118$^{**}$ & $-$0.124$^{**}$ \\ 
  & (0.041) & (0.042) & (0.048) & (0.048) \\ 
  lag(Ban gatherings, 21) & $-$0.157$^{***}$ & $-$0.158$^{**}$ & $-$0.165$^{***}$ & $-$0.164$^{**}$ \\ 
  & (0.053) & (0.072) & (0.050) & (0.068) \\ 
  lag(Stay at Staying Home Devices, 21) & $-$0.215$^{***}$ & $-$0.219$^{***}$ & $-$0.232$^{***}$ & $-$0.233$^{***}$ \\ 
  & (0.050) & (0.047) & (0.052) & (0.048) \\ 
  lag(College Visits, 21) & 0.155 & 0.106 & 0.008 & 0.046 \\ 
  & (0.140) & (0.144) & (0.149) & (0.150) \\ 
  lag(K-12 School Visits, 21) & 0.876$^{***}$ & 0.919$^{***}$ &  &  \\ 
  & (0.169) & (0.196) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 21) &  & 0.090 &  &  \\ 
  &  & (0.117) &  &  \\ 
  lag(Open K-12 In-person, 21) &  &  & 0.039 & 0.044 \\ 
  &  &  & (0.046) & (0.062) \\ 
  lag(Open K-12 Hybrid, 21) &  &  & 0.018 & 0.014 \\ 
  &  &  & (0.030) & (0.031) \\ 
  lag(Open K-12 Remote, 21) &  &  & 0.005 & $-$0.006 \\ 
  &  &  & (0.036) & (0.037) \\ 
  lag(full\_staff\_dum, 21) &  &  &  & $-$0.016 \\ 
  &  &  &  & (0.041) \\ 
  lag(hybrid\_staff\_dum, 21) &  &  &  & 0.008 \\ 
  &  &  &  & (0.036) \\ 
  lag(const, 21) &  &  &  &  \\ 
  &  &  &  &  \\ 
  Test Growth Rates & 0.003$^{**}$ & 0.002$^{*}$ & 0.003$^{**}$ & 0.002$^{**}$ \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 677,246 & 535,590 & 601,512 & 519,743 \\ 
R$^{2}$ & 0.159 & 0.155 & 0.156 & 0.155 \\ 
Adjusted R$^{2}$ & 0.153 & 0.148 & 0.149 & 0.148 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt4-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.033$^{**}$ & $-$0.025 & $-$0.030$^{*}$ & $-$0.032$^{**}$ \\ 
  & (0.015) & (0.015) & (0.016) & (0.016) \\ 
  lag(Ban gatherings, 14) & $-$0.009 & $-$0.009 & $-$0.015 & $-$0.012 \\ 
  & (0.047) & (0.055) & (0.046) & (0.053) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.117$^{***}$ & $-$0.118$^{***}$ & $-$0.121$^{***}$ & $-$0.126$^{***}$ \\ 
  & (0.036) & (0.037) & (0.037) & (0.037) \\ 
  lag(College Visits, 14) & 0.167$^{**}$ & 0.192$^{**}$ & 0.134$^{**}$ & 0.177$^{**}$ \\ 
  & (0.069) & (0.085) & (0.064) & (0.075) \\ 
  lag(K-12 School Visits, 14) & 0.307$^{***}$ & 0.384$^{***}$ &  &  \\ 
  & (0.099) & (0.106) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & $-$0.051 &  &  \\ 
  &  & (0.101) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & $-$0.003 & 0.003 \\ 
  &  &  & (0.017) & (0.017) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.010 & 0.011 \\ 
  &  &  & (0.015) & (0.015) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.001 & $-$0.006 \\ 
  &  &  & (0.018) & (0.018) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & $-$0.046$^{*}$ \\ 
  &  &  &  & (0.026) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & $-$0.005 \\ 
  &  &  &  & (0.019) \\ 
  lag(const, 14) &  &  &  &  \\ 
  &  &  &  &  \\ 
  Test Growth Rates & 0.008 & 0.007 & 0.008 & 0.007 \\ 
  & (0.006) & (0.006) & (0.006) & (0.006) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 584,371 & 452,585 & 514,806 & 439,202 \\ 
R$^{2}$ & 0.087 & 0.088 & 0.087 & 0.088 \\ 
Adjusted R$^{2}$ & 0.080 & 0.080 & 0.080 & 0.080 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-alt5-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & 0.024$^{***}$ & 0.032$^{***}$ & 0.024$^{***}$ & 0.029$^{***}$ \\ 
  & (0.007) & (0.008) & (0.008) & (0.009) \\ 
  lag(Ban gatherings, 14) & $-$0.001 & 0.0001 & $-$0.002 & $-$0.001 \\ 
  & (0.026) & (0.032) & (0.025) & (0.031) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.133$^{***}$ & $-$0.125$^{***}$ & $-$0.133$^{***}$ & $-$0.133$^{***}$ \\ 
  & (0.038) & (0.043) & (0.040) & (0.044) \\ 
  lag(College Visits, 14) & 0.256$^{***}$ & 0.276$^{***}$ & 0.235$^{***}$ & 0.260$^{***}$ \\ 
  & (0.054) & (0.065) & (0.050) & (0.060) \\ 
  lag(K-12 School Visits, 14) & 0.080 & 0.117$^{**}$ &  &  \\ 
  & (0.053) & (0.050) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & $-$0.003 &  &  \\ 
  &  & (0.029) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & $-$0.037$^{**}$ & $-$0.037$^{**}$ \\ 
  &  &  & (0.014) & (0.017) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & $-$0.010 & $-$0.013 \\ 
  &  &  & (0.010) & (0.012) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.004 & $-$0.0001 \\ 
  &  &  & (0.012) & (0.013) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & $-$0.008 \\ 
  &  &  &  & (0.016) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.007 \\ 
  &  &  &  & (0.010) \\ 
  lag(log(Cases), 14) & $-$0.037$^{***}$ & $-$0.040$^{***}$ & $-$0.037$^{***}$ & $-$0.040$^{***}$ \\ 
  & (0.007) & (0.008) & (0.008) & (0.008) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.015$^{***}$ & $-$0.014$^{***}$ & $-$0.015$^{***}$ & $-$0.014$^{**}$ \\ 
  & (0.004) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & 0.014$^{***}$ & 0.014$^{***}$ & 0.013$^{***}$ & 0.012$^{***}$ \\ 
  & (0.004) & (0.003) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{*}$ & 0.009 & 0.010$^{*}$ & 0.009 \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,108 & 544,980 & 612,771 & 528,790 \\ 
R$^{2}$ & 0.078 & 0.077 & 0.077 & 0.077 \\ 
Adjusted R$^{2}$ & 0.075 & 0.074 & 0.074 & 0.074 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-fe-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.006 & $-$0.006 & $-$0.015 & $-$0.017 \\ 
  & (0.018) & (0.017) & (0.020) & (0.019) \\ 
  lag(Ban gatherings, 14) & $-$0.066$^{*}$ & $-$0.068 & $-$0.068$^{**}$ & $-$0.067 \\ 
  & (0.033) & (0.044) & (0.033) & (0.042) \\ 
  lag(Stay at home, 14) & $-$0.203$^{***}$ & $-$0.198$^{***}$ & $-$0.200$^{***}$ & $-$0.200$^{***}$ \\ 
  & (0.031) & (0.039) & (0.034) & (0.040) \\ 
  lag(College Visits, 14) & 0.359$^{***}$ & 0.412$^{***}$ & 0.326$^{***}$ & 0.371$^{***}$ \\ 
  & (0.071) & (0.073) & (0.064) & (0.076) \\ 
  lag(K-12 Visits, 14) & 0.393$^{***}$ & 0.429$^{***}$ &  &  \\ 
  & (0.070) & (0.070) &  &  \\ 
  lag(K-12 Visits\_staff\_dum, 14) &  & 0.100 &  &  \\ 
  &  & (0.070) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.062$^{***}$ & 0.062$^{***}$ \\ 
  &  &  & (0.017) & (0.021) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.040$^{***}$ & 0.033$^{**}$ \\ 
  &  &  & (0.014) & (0.013) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.030$^{*}$ & 0.027$^{*}$ \\ 
  &  &  & (0.016) & (0.015) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.009 \\ 
  &  &  &  & (0.019) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.032$^{*}$ \\ 
  &  &  &  & (0.017) \\ 
  lag(log(Cases), 14d lag, 14) & $-$0.088$^{***}$ & $-$0.092$^{***}$ & $-$0.088$^{***}$ & $-$0.092$^{***}$ \\ 
  & (0.009) & (0.010) & (0.010) & (0.010) \\ 
  lag(lag(log(Cases), 14d lag, 7), 14) & $-$0.042$^{***}$ & $-$0.043$^{***}$ & $-$0.043$^{***}$ & $-$0.043$^{***}$ \\ 
  & (0.005) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14d lag, 14), 14) & $-$0.017$^{***}$ & $-$0.020$^{***}$ & $-$0.018$^{***}$ & $-$0.021$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{**}$ & 0.008$^{*}$ & 0.009$^{**}$ & 0.009$^{*}$ \\ 
  & (0.004) & (0.004) & (0.004) & (0.004) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,297 & 545,131 & 612,963 & 528,941 \\ 
R$^{2}$ & 0.092 & 0.093 & 0.092 & 0.094 \\ 
Adjusted R$^{2}$ & 0.085 & 0.086 & 0.085 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-fulltime-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{fullwork} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.003$^{***}$ & $-$0.004$^{***}$ \\ 
  & (0.0005) & (0.001) \\ 
  lag(Ban gatherings >50, 14) & 0.002$^{**}$ & 0.002$^{**}$ \\ 
  & (0.001) & (0.001) \\ 
  lag(Stay at home, 14) & 0.003$^{***}$ & 0.003$^{***}$ \\ 
  & (0.001) & (0.001) \\ 
  lag(College Visits, 14) & $-$0.099$^{***}$ & $-$0.110$^{***}$ \\ 
  & (0.004) & (0.005) \\ 
  lag(K-12 Visits, 14) & 0.082$^{***}$ &  \\ 
  & (0.005) &  \\ 
  lag(Open K-12 full, 14) &  & 0.011$^{***}$ \\ 
  &  & (0.001) \\ 
  lag(Open K-12 hybrid, 14) &  & 0.002$^{***}$ \\ 
  &  & (0.0003) \\ 
  lag(Open K-12 remote, 14) &  & $-$0.002$^{***}$ \\ 
  &  & (0.0005) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.00001 & 0.00001 \\ 
  & (0.00004) & (0.00005) \\ 
  lag(lag($\log \Delta C_{it}$, 7), 14) & 0.00003 & $-$0.00002 \\ 
  & (0.00003) & (0.00004) \\ 
  lag(lag($\log \Delta C_{it}$, 14), 14) & 0.00001 & 0.00002 \\ 
  & (0.00003) & (0.00004) \\ 
  $\Delta \log T_{it}$ & 0.0001$^{**}$ & 0.0001$^{**}$ \\ 
  & (0.00004) & (0.00004) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes \\ 
state & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 645,220 & 602,393 \\ 
R$^{2}$ & 0.847 & 0.837 \\ 
Adjusted R$^{2}$ & 0.846 & 0.836 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-mask-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
 & \multicolumn{2}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.107$^{***}$ & $-$0.134$^{***}$ \\ 
  & (0.015) & (0.019) \\ 
  lag(Ban gatherings, 14) & $-$0.124$^{***}$ & $-$0.135$^{***}$ \\ 
  & (0.033) & (0.034) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.263$^{***}$ & $-$0.262$^{***}$ \\ 
  & (0.032) & (0.034) \\ 
  lag(College Visits, 14) & 0.140$^{**}$ & 0.132$^{**}$ \\ 
  & (0.071) & (0.064) \\ 
  lag(K-12 School Visits, 14) & 0.514$^{***}$ &  \\ 
  & (0.095) &  \\ 
  lag(K-12 School Visits\_Mandatory mask, 14) & $-$0.109 &  \\ 
  & (0.163) &  \\ 
  lag(Open K-12 In-person, 14) &  & 0.027 \\ 
  &  & (0.022) \\ 
  lag(Open K-12 Hybrid, 14) &  & $-$0.001 \\ 
  &  & (0.018) \\ 
  lag(Open K-12 Remote, 14) &  & $-$0.081$^{***}$ \\ 
  &  & (0.015) \\ 
  lag(full\_Mandatory mask, 14) &  & 0.034 \\ 
  &  & (0.027) \\ 
  lag(hybrid\_Mandatory mask, 14) &  & $-$0.010 \\ 
  &  & (0.014) \\ 
  lag(log(Cases), 14) & $-$0.101$^{***}$ & $-$0.098$^{***}$ \\ 
  & (0.009) & (0.010) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.061$^{***}$ & $-$0.060$^{***}$ \\ 
  & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.030$^{***}$ & $-$0.031$^{***}$ \\ 
  & (0.003) & (0.004) \\ 
  Test Growth Rates & 0.009$^{**}$ & 0.009$^{**}$ \\ 
  & (0.004) & (0.004) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes \\ 
state & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,297 & 612,963 \\ 
R$^{2}$ & 0.092 & 0.092 \\ 
Adjusted R$^{2}$ & 0.085 & 0.085 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-pbiy-pbiy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.006 & $-$0.006 & $-$0.015 & $-$0.017 \\ 
  & (0.018) & (0.017) & (0.019) & (0.019) \\ 
  lag(Ban gatherings >50, 14) & $-$0.066$^{*}$ & $-$0.065 & $-$0.064$^{*}$ & $-$0.061 \\ 
  & (0.034) & (0.044) & (0.034) & (0.043) \\ 
  lag(Stay at home, 14) & $-$0.197$^{***}$ & $-$0.188$^{***}$ & $-$0.187$^{***}$ & $-$0.184$^{***}$ \\ 
  & (0.033) & (0.040) & (0.034) & (0.040) \\ 
  lag(College Visits, 14) & 0.322$^{***}$ & 0.383$^{***}$ & 0.320$^{***}$ & 0.374$^{***}$ \\ 
  & (0.071) & (0.072) & (0.065) & (0.075) \\ 
  lag(K-12 Visits, 14) & 0.431$^{***}$ & 0.425$^{***}$ &  &  \\ 
  & (0.075) & (0.087) &  &  \\ 
  lag(K-12 Visits\_staff\_dum, 14) &  & 0.091 &  &  \\ 
  &  & (0.071) &  &  \\ 
  lag(Open K-12 full, 14) &  &  & 0.051$^{***}$ & 0.049$^{**}$ \\ 
  &  &  & (0.016) & (0.020) \\ 
  lag(Open K-12 hybrid, 14) &  &  & 0.034$^{**}$ & 0.025$^{**}$ \\ 
  &  &  & (0.013) & (0.013) \\ 
  lag(Open K-12 remote, 14) &  &  & 0.026$^{*}$ & 0.020 \\ 
  &  &  & (0.015) & (0.014) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.005 \\ 
  &  &  &  & (0.020) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.030$^{*}$ \\ 
  &  &  &  & (0.017) \\ 
  lag(fullwork, 14) & 0.041 & 0.219 & 0.672$^{*}$ & 0.732$^{*}$ \\ 
  & (0.417) & (0.490) & (0.384) & (0.436) \\ 
  lag(partwork, 14) & $-$0.433 & $-$0.185 & $-$0.070 & 0.116 \\ 
  & (0.259) & (0.305) & (0.276) & (0.309) \\ 
  lag(home, 14) & $-$0.184$^{***}$ & $-$0.209$^{***}$ & $-$0.230$^{***}$ & $-$0.244$^{***}$ \\ 
  & (0.057) & (0.069) & (0.061) & (0.067) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.087$^{***}$ & $-$0.091$^{***}$ & $-$0.087$^{***}$ & $-$0.092$^{***}$ \\ 
  & (0.009) & (0.010) & (0.010) & (0.010) \\ 
  lag(lag($\log \Delta C_{it}$, 7), 14) & $-$0.042$^{***}$ & $-$0.043$^{***}$ & $-$0.042$^{***}$ & $-$0.043$^{***}$ \\ 
  & (0.004) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag($\log \Delta C_{it}$, 14), 14) & $-$0.017$^{***}$ & $-$0.019$^{***}$ & $-$0.018$^{***}$ & $-$0.021$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) & (0.003) \\ 
  $\Delta \log T_{it}$ & 0.009$^{**}$ & 0.008$^{*}$ & 0.009$^{**}$ & 0.009$^{*}$ \\ 
  & (0.004) & (0.004) & (0.004) & (0.004) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,297 & 545,131 & 612,963 & 528,941 \\ 
R$^{2}$ & 0.092 & 0.093 & 0.092 & 0.094 \\ 
Adjusted R$^{2}$ & 0.085 & 0.086 & 0.085 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-pbiy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.008 & $-$0.008 & $-$0.017 & $-$0.019 \\ 
  & (0.017) & (0.017) & (0.019) & (0.019) \\ 
  lag(Ban gatherings, 14) & $-$0.066$^{*}$ & $-$0.063 & $-$0.058 & $-$0.059 \\ 
  & (0.036) & (0.046) & (0.035) & (0.044) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.198$^{***}$ & $-$0.189$^{***}$ & $-$0.188$^{***}$ & $-$0.186$^{***}$ \\ 
  & (0.033) & (0.039) & (0.035) & (0.039) \\ 
  lag(College Visits, 14) & 0.309$^{***}$ & 0.378$^{***}$ & 0.306$^{***}$ & 0.370$^{***}$ \\ 
  & (0.071) & (0.073) & (0.066) & (0.076) \\ 
  lag(K-12 School Visits, 14) & 0.431$^{***}$ & 0.418$^{***}$ &  &  \\ 
  & (0.076) & (0.087) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.100 &  &  \\ 
  &  & (0.071) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.052$^{***}$ & 0.048$^{**}$ \\ 
  &  &  & (0.016) & (0.020) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.034$^{**}$ & 0.025$^{*}$ \\ 
  &  &  & (0.013) & (0.013) \\ 
  lag(Open K-12 Remote, 14) &  &  & 0.025 & 0.019 \\ 
  &  &  & (0.015) & (0.014) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.007 \\ 
  &  &  &  & (0.020) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.031$^{*}$ \\ 
  &  &  &  & (0.017) \\ 
  lag(Full-time Workplace Visits, 14) & 0.137 & 0.300 & 0.728$^{*}$ & 0.809$^{*}$ \\ 
  & (0.399) & (0.472) & (0.371) & (0.422) \\ 
  lag(Part-time Workplace Visits, 14) & $-$0.461$^{*}$ & $-$0.161 & $-$0.076 & 0.143 \\ 
  & (0.264) & (0.312) & (0.286) & (0.315) \\ 
  lag(Staying Home Devices, 14) & $-$0.181$^{***}$ & $-$0.207$^{***}$ & $-$0.232$^{***}$ & $-$0.243$^{***}$ \\ 
  & (0.057) & (0.070) & (0.060) & (0.067) \\ 
  lag(log(Cases), 14) & $-$0.087$^{***}$ & $-$0.091$^{***}$ & $-$0.087$^{***}$ & $-$0.092$^{***}$ \\ 
  & (0.009) & (0.010) & (0.010) & (0.010) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.042$^{***}$ & $-$0.043$^{***}$ & $-$0.043$^{***}$ & $-$0.043$^{***}$ \\ 
  & (0.004) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.017$^{***}$ & $-$0.019$^{***}$ & $-$0.018$^{***}$ & $-$0.021$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{*}$ & 0.009 & 0.010$^{*}$ & 0.009 \\ 
  & (0.005) & (0.006) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,108 & 544,980 & 612,771 & 528,790 \\ 
R$^{2}$ & 0.092 & 0.093 & 0.092 & 0.094 \\ 
Adjusted R$^{2}$ & 0.085 & 0.086 & 0.085 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.115$^{***}$ & $-$0.125$^{***}$ & $-$0.131$^{***}$ & $-$0.130$^{***}$ \\ 
  & (0.018) & (0.017) & (0.019) & (0.019) \\ 
  lag(Ban gatherings, 14) & $-$0.141$^{***}$ & $-$0.144$^{***}$ & $-$0.142$^{***}$ & $-$0.145$^{***}$ \\ 
  & (0.036) & (0.045) & (0.035) & (0.044) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.262$^{***}$ & $-$0.260$^{***}$ & $-$0.261$^{***}$ & $-$0.267$^{***}$ \\ 
  & (0.032) & (0.039) & (0.034) & (0.039) \\ 
  lag(College Visits, 14) & 0.130$^{*}$ & 0.060 & 0.121$^{*}$ & 0.001 \\ 
  & (0.072) & (0.075) & (0.067) & (0.079) \\ 
  lag(K-12 School Visits, 14) & 0.481$^{***}$ & 0.399$^{***}$ &  &  \\ 
  & (0.071) & (0.072) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.299$^{***}$ &  &  \\ 
  &  & (0.071) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.048$^{***}$ & 0.024 \\ 
  &  &  & (0.017) & (0.021) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & $-$0.008 & $-$0.037$^{***}$ \\ 
  &  &  & (0.014) & (0.014) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.082$^{***}$ & $-$0.102$^{***}$ \\ 
  &  &  & (0.015) & (0.015) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.045$^{**}$ \\ 
  &  &  &  & (0.019) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.051$^{***}$ \\ 
  &  &  &  & (0.017) \\ 
  lag(log(Cases), 14) & $-$0.101$^{***}$ & $-$0.101$^{***}$ & $-$0.098$^{***}$ & $-$0.099$^{***}$ \\ 
  & (0.009) & (0.010) & (0.010) & (0.010) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.061$^{***}$ & $-$0.060$^{***}$ & $-$0.060$^{***}$ & $-$0.060$^{***}$ \\ 
  & (0.005) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.030$^{***}$ & $-$0.033$^{***}$ & $-$0.031$^{***}$ & $-$0.034$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{*}$ & 0.009 & 0.010$^{*}$ & 0.009$^{*}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,108 & 544,980 & 612,771 & 528,790 \\ 
R$^{2}$ & 0.092 & 0.093 & 0.092 & 0.094 \\ 
Adjusted R$^{2}$ & 0.085 & 0.086 & 0.085 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-selection-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
 & \multicolumn{3}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.088$^{***}$ & $-$0.095$^{***}$ & $-$0.101$^{***}$ \\ 
  & (0.021) & (0.020) & (0.020) \\ 
  lag(Ban gatherings, 14) & $-$0.137$^{***}$ & $-$0.150$^{***}$ & $-$0.149$^{***}$ \\ 
  & (0.032) & (0.043) & (0.032) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.266$^{***}$ & $-$0.257$^{***}$ & $-$0.247$^{***}$ \\ 
  & (0.032) & (0.041) & (0.034) \\ 
  lag(College Visits, 14) & 0.422$^{***}$ & 0.423$^{***}$ & 0.357$^{***}$ \\ 
  & (0.073) & (0.074) & (0.064) \\ 
  lag(K-12 School Visits, 14) & 0.607$^{***}$ & 0.433$^{**}$ &  \\ 
  & (0.175) & (0.202) &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.449$^{***}$ &  \\ 
  &  & (0.084) &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.163$^{***}$ \\ 
  &  &  & (0.016) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & 0.031$^{**}$ \\ 
  &  &  & (0.013) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.063$^{***}$ \\ 
  &  &  & (0.015) \\ 
  lag(log(Cases), 14) & $-$0.096$^{***}$ & $-$0.093$^{***}$ & $-$0.093$^{***}$ \\ 
  & (0.010) & (0.010) & (0.011) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.060$^{***}$ & $-$0.059$^{***}$ & $-$0.060$^{***}$ \\ 
  & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.031$^{***}$ & $-$0.032$^{***}$ & $-$0.031$^{***}$ \\ 
  & (0.003) & (0.003) & (0.003) \\ 
  Test Growth Rates & 0.007 & 0.006 & 0.007 \\ 
  & (0.005) & (0.005) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 760,422 & 600,958 & 675,405 \\ 
R$^{2}$ & 0.092 & 0.094 & 0.092 \\ 
Adjusted R$^{2}$ & 0.086 & 0.086 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases2-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Case Growth Rates} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 14) & $-$0.114$^{***}$ & $-$0.126$^{***}$ & $-$0.130$^{***}$ & $-$0.132$^{***}$ \\ 
  & (0.018) & (0.017) & (0.020) & (0.019) \\ 
  lag(Ban gatherings, 14) & $-$0.124$^{***}$ & $-$0.137$^{***}$ & $-$0.135$^{***}$ & $-$0.139$^{***}$ \\ 
  & (0.033) & (0.044) & (0.033) & (0.042) \\ 
  lag(Stay at Staying Home Devices, 14) & $-$0.264$^{***}$ & $-$0.261$^{***}$ & $-$0.261$^{***}$ & $-$0.268$^{***}$ \\ 
  & (0.031) & (0.039) & (0.034) & (0.040) \\ 
  lag(College Visits, 14) & 0.150$^{**}$ & 0.085 & 0.144$^{**}$ & 0.025 \\ 
  & (0.071) & (0.073) & (0.064) & (0.076) \\ 
  lag(K-12 School Visits, 14) & 0.453$^{***}$ & 0.372$^{***}$ &  &  \\ 
  & (0.070) & (0.070) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 14) &  & 0.282$^{***}$ &  &  \\ 
  &  & (0.070) &  &  \\ 
  lag(Open K-12 In-person, 14) &  &  & 0.048$^{***}$ & 0.025 \\ 
  &  &  & (0.017) & (0.021) \\ 
  lag(Open K-12 Hybrid, 14) &  &  & $-$0.012 & $-$0.042$^{***}$ \\ 
  &  &  & (0.014) & (0.013) \\ 
  lag(Open K-12 Remote, 14) &  &  & $-$0.081$^{***}$ & $-$0.100$^{***}$ \\ 
  &  &  & (0.016) & (0.015) \\ 
  lag(full\_staff\_dum, 14) &  &  &  & 0.036$^{*}$ \\ 
  &  &  &  & (0.019) \\ 
  lag(hybrid\_staff\_dum, 14) &  &  &  & 0.053$^{***}$ \\ 
  &  &  &  & (0.017) \\ 
  lag(log(Cases), 14) & $-$0.101$^{***}$ & $-$0.102$^{***}$ & $-$0.098$^{***}$ & $-$0.099$^{***}$ \\ 
  & (0.009) & (0.010) & (0.010) & (0.010) \\ 
  lag(lag(log(Cases), 7), 14) & $-$0.061$^{***}$ & $-$0.060$^{***}$ & $-$0.060$^{***}$ & $-$0.059$^{***}$ \\ 
  & (0.005) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Cases), 14), 14) & $-$0.031$^{***}$ & $-$0.033$^{***}$ & $-$0.031$^{***}$ & $-$0.034$^{***}$ \\ 
  & (0.003) & (0.003) & (0.004) & (0.004) \\ 
  Test Growth Rates & 0.009$^{**}$ & 0.008$^{*}$ & 0.009$^{**}$ & 0.009$^{**}$ \\ 
  & (0.004) & (0.004) & (0.004) & (0.004) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 690,297 & 545,131 & 612,963 & 528,941 \\ 
R$^{2}$ & 0.092 & 0.093 & 0.092 & 0.094 \\ 
Adjusted R$^{2}$ & 0.085 & 0.086 & 0.085 & 0.086 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/corr-mitigation-hybrid.tex <==

\begin{tabular}{lcccc}
\toprule
\rotatebox{90}{ } & \rotatebox{90}{No mask for staffs} & \rotatebox{90}{No mask for students} & \rotatebox{90}{Yes sports for students} & \rotatebox{90}{character(0)}\\
\midrule
No mask for staffs & 1.00 &  &  & \\
No mask for students & 0.73 & 1.00 &  & \\
Yes sports for students & 0.16 & 0.14 & 1.00 & \\
character(0) & 0.11 & 0.08 & 0.02 & 1.00\\
\bottomrule
\end{tabular}

==> tables_and_figures/corr-mitigation.tex <==

\begin{tabular}{lcccc}
\toprule
\rotatebox{90}{ } & \rotatebox{90}{No mask for staffs} & \rotatebox{90}{No mask for students} & \rotatebox{90}{Yes sports for students} & \rotatebox{90}{No online instruction}\\
\midrule
No mask for staffs & 1.00 &  &  & \\
No mask for students & 0.736^{***} & 1.00 &  & \\
Yes sports for students & 0.14^{***}  & 0.07^{***}  & 1.00 & \\
No online instruction & 0.13^{***}  & 0.12^{***}  & 0.06^{**}  & 1.00\\
\bottomrule
\end{tabular}

==> tables_and_figures/corr.tex <==

\begin{tabular}{lcccccccccccccccc}
\toprule
\rotatebox{90}{ } & \rotatebox{90}{College Visits} & \rotatebox{90}{K-12 School Visits} & \rotatebox{90}{Open K-12 In-person} & \rotatebox{90}{Open K-12 Hybrid} & \rotatebox{90}{Open K-12 Remote} & \rotatebox{90}{No-Mask for Staffs} & \rotatebox{90}{Mandatory mask} & \rotatebox{90}{Ban gatherings} & \rotatebox{90}{Stay at home} & \rotatebox{90}{Full-time Workplace Visits} & \rotatebox{90}{Part-time Workplace Visits} & \rotatebox{90}{Staying Home Devices} & \rotatebox{90}{Bar Visits} & \rotatebox{90}{Restaurant Visits} & \rotatebox{90}{Rec. Facilities Visits} & \rotatebox{90}{Church Vists}\\
\midrule
College Visits & 1.00 &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
K-12 School Visits & 0.09 & 1.00 &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
Open K-12 In-person & 0.05 & 0.43 & 1.00 &  &  &  &  &  &  &  &  &  &  &  &  & \\
Open K-12 Hybrid & 0.11 & 0.44 & 0.04 & 1.00 &  &  &  &  &  &  &  &  &  &  &  & \\
Open K-12 Remote & 0.05 & 0.09 & -0.06 & -0.06 & 1.00 &  &  &  &  &  &  &  &  &  &  & \\
\addlinespace
No-Mask for Staffs & 0.01 & 0.16 & 0.15 & -0.02 & -0.10 & 1.00 &  &  &  &  &  &  &  &  &  & \\
Mandatory mask & 0.09 & 0.10 & 0.03 & 0.24 & 0.23 & -0.31 & 1.00 &  &  &  &  &  &  &  &  & \\
Ban gatherings & -0.03 & -0.14 & -0.09 & -0.06 & 0.00 & -0.03 & -0.09 & 1.00 &  &  &  &  &  &  &  & \\
Stay at home & -0.06 & -0.24 & -0.14 & -0.21 & -0.13 & -0.08 & -0.19 & 0.20 & 1.00 &  &  &  &  &  &  & \\
Full-time Workplace Visits & 0.04 & 0.56 & 0.37 & 0.36 & 0.10 & 0.12 & 0.05 & -0.17 & -0.21 & 1.00 &  &  &  &  &  & \\
\addlinespace
Part-time Workplace Visits & 0.06 & 0.60 & 0.32 & 0.34 & 0.04 & 0.20 & -0.01 & -0.12 & -0.31 & 0.71 & 1.00 &  &  &  &  & \\
Staying Home Devices & -0.04 & -0.27 & -0.18 & -0.23 & -0.02 & -0.10 & 0.01 & -0.00 & 0.27 & 0.06 & -0.19 & 1.00 &  &  &  & \\
Bar Visits & 0.05 & 0.08 & 0.02 & -0.02 & 0.01 & 0.08 & 0.01 & -0.06 & -0.08 & 0.12 & 0.11 & 0.15 & 1.00 &  &  & \\
Restaurant Visits & 0.17 & 0.02 & -0.10 & 0.00 & 0.06 & -0.10 & 0.14 & 0.10 & -0.08 & -0.07 & 0.07 & 0.04 & 0.34 & 1.00 &  & \\
Rec. Facilities Visits & 0.15 & -0.00 & -0.07 & 0.03 & 0.11 & -0.08 & 0.18 & 0.03 & -0.08 & -0.05 & -0.03 & 0.09 & 0.26 & 0.52 & 1.00 & \\
\addlinespace
Church Vists & 0.06 & 0.32 & 0.13 & 0.08 & -0.03 & 0.17 & -0.06 & -0.07 & -0.16 & 0.15 & 0.37 & -0.18 & 0.11 & 0.18 & 0.03 & 1.00\\
\bottomrule
\end{tabular}

==> tables_and_figures/deaths-alt-fulltime35-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d3log(Deaths)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 35) & $-$0.125$^{***}$ & $-$0.123$^{***}$ & $-$0.139$^{***}$ & $-$0.124$^{***}$ \\ 
  & (0.027) & (0.025) & (0.027) & (0.026) \\ 
  lag(Ban gatherings, 35) & $-$0.218$^{***}$ & $-$0.356$^{***}$ & $-$0.291$^{***}$ & $-$0.358$^{***}$ \\ 
  & (0.079) & (0.096) & (0.081) & (0.097) \\ 
  lag(Stay at Staying Home Devices, 35) & $-$0.207$^{***}$ & $-$0.143$^{**}$ & $-$0.155$^{**}$ & $-$0.125$^{*}$ \\ 
  & (0.058) & (0.064) & (0.062) & (0.069) \\ 
  lag(College Visits, 35) & 0.331$^{*}$ & 0.590$^{***}$ & 0.625$^{***}$ & 0.706$^{***}$ \\ 
  & (0.196) & (0.199) & (0.199) & (0.192) \\ 
  lag(K-12 School Visits, 35) & 0.494$^{***}$ & 0.270 &  &  \\ 
  & (0.121) & (0.168) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 35) &  & 0.622$^{***}$ &  &  \\ 
  &  & (0.221) &  &  \\ 
  lag(Open K-12 In-person, 35) &  &  & $-$0.018 & 0.024 \\ 
  &  &  & (0.050) & (0.060) \\ 
  lag(Open K-12 Hybrid, 35) &  &  & $-$0.019 & $-$0.052$^{*}$ \\ 
  &  &  & (0.027) & (0.028) \\ 
  lag(Open K-12 Remote, 35) &  &  & $-$0.055$^{*}$ & $-$0.105$^{***}$ \\ 
  &  &  & (0.030) & (0.039) \\ 
  lag(full\_staff\_dum, 35) &  &  &  & 0.056 \\ 
  &  &  &  & (0.068) \\ 
  lag(hybrid\_staff\_dum, 35) &  &  &  & 0.131$^{**}$ \\ 
  &  &  &  & (0.051) \\ 
  lag(log(Deaths), 35) & $-$0.665$^{***}$ & $-$0.675$^{***}$ & $-$0.661$^{***}$ & $-$0.672$^{***}$ \\ 
  & (0.013) & (0.013) & (0.013) & (0.013) \\ 
  lag(lag(log(Deaths), 7), 35) & $-$0.046$^{***}$ & $-$0.050$^{***}$ & $-$0.044$^{***}$ & $-$0.049$^{***}$ \\ 
  & (0.006) & (0.006) & (0.007) & (0.007) \\ 
  lag(lag(log(Deaths), 14), 35) & $-$0.061$^{***}$ & $-$0.064$^{***}$ & $-$0.058$^{***}$ & $-$0.063$^{***}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
  lag(Full-time Workplace Visits, 35) & $-$1.803$^{***}$ & $-$2.080$^{***}$ & 0.033 & $-$0.711 \\ 
  & (0.668) & (0.642) & (0.700) & (0.690) \\ 
  lag(Part-time Workplace Visits, 35) & 2.041$^{***}$ & 1.920$^{***}$ & 2.162$^{***}$ & 2.325$^{***}$ \\ 
  & (0.487) & (0.552) & (0.499) & (0.492) \\ 
  lag(Staying Home Devices, 35) & 0.412$^{***}$ & 0.531$^{***}$ & 0.383$^{***}$ & 0.559$^{***}$ \\ 
  & (0.109) & (0.099) & (0.116) & (0.097) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 615,523 & 485,776 & 546,519 & 471,386 \\ 
R$^{2}$ & 0.268 & 0.274 & 0.273 & 0.276 \\ 
Adjusted R$^{2}$ & 0.262 & 0.268 & 0.267 & 0.270 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-alt35-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d3log(Deaths)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 35) & $-$0.127$^{***}$ & $-$0.125$^{***}$ & $-$0.142$^{***}$ & $-$0.123$^{***}$ \\ 
  & (0.027) & (0.024) & (0.027) & (0.025) \\ 
  lag(Ban gatherings, 35) & $-$0.212$^{***}$ & $-$0.355$^{***}$ & $-$0.292$^{***}$ & $-$0.360$^{***}$ \\ 
  & (0.077) & (0.094) & (0.080) & (0.095) \\ 
  lag(Stay at Staying Home Devices, 35) & $-$0.198$^{***}$ & $-$0.127$^{**}$ & $-$0.156$^{**}$ & $-$0.116$^{*}$ \\ 
  & (0.057) & (0.064) & (0.062) & (0.069) \\ 
  lag(College Visits, 35) & 0.313 & 0.530$^{***}$ & 0.507$^{***}$ & 0.561$^{***}$ \\ 
  & (0.199) & (0.203) & (0.196) & (0.193) \\ 
  lag(K-12 School Visits, 35) & 0.648$^{***}$ & 0.329$^{**}$ &  &  \\ 
  & (0.113) & (0.165) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 35) &  & 0.617$^{***}$ &  &  \\ 
  &  & (0.222) &  &  \\ 
  lag(Open K-12 In-person, 35) &  &  & 0.015 & 0.040 \\ 
  &  &  & (0.052) & (0.063) \\ 
  lag(Open K-12 Hybrid, 35) &  &  & 0.004 & $-$0.041 \\ 
  &  &  & (0.027) & (0.028) \\ 
  lag(Open K-12 Remote, 35) &  &  & $-$0.048 & $-$0.109$^{***}$ \\ 
  &  &  & (0.030) & (0.040) \\ 
  lag(full\_staff\_dum, 35) &  &  &  & 0.050 \\ 
  &  &  &  & (0.068) \\ 
  lag(hybrid\_staff\_dum, 35) &  &  &  & 0.141$^{***}$ \\ 
  &  &  &  & (0.050) \\ 
  lag(log(Deaths), 35) & $-$0.666$^{***}$ & $-$0.675$^{***}$ & $-$0.662$^{***}$ & $-$0.672$^{***}$ \\ 
  & (0.013) & (0.013) & (0.013) & (0.013) \\ 
  lag(lag(log(Deaths), 7), 35) & $-$0.047$^{***}$ & $-$0.050$^{***}$ & $-$0.045$^{***}$ & $-$0.049$^{***}$ \\ 
  & (0.006) & (0.007) & (0.007) & (0.007) \\ 
  lag(lag(log(Deaths), 14), 35) & $-$0.062$^{***}$ & $-$0.064$^{***}$ & $-$0.059$^{***}$ & $-$0.063$^{***}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 615,523 & 485,776 & 546,519 & 471,386 \\ 
R$^{2}$ & 0.268 & 0.274 & 0.273 & 0.276 \\ 
Adjusted R$^{2}$ & 0.262 & 0.267 & 0.267 & 0.269 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-fulltime35-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d3log(Deaths)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 35) & $-$0.129$^{***}$ & $-$0.105$^{***}$ & $-$0.135$^{***}$ & $-$0.105$^{***}$ \\ 
  & (0.027) & (0.025) & (0.028) & (0.026) \\ 
  lag(Ban gatherings, 35) & $-$0.264$^{***}$ & $-$0.360$^{***}$ & $-$0.336$^{***}$ & $-$0.364$^{***}$ \\ 
  & (0.075) & (0.099) & (0.080) & (0.100) \\ 
  lag(Stay at Staying Home Devices, 35) & $-$0.210$^{***}$ & $-$0.147$^{**}$ & $-$0.157$^{**}$ & $-$0.128$^{*}$ \\ 
  & (0.059) & (0.066) & (0.065) & (0.072) \\ 
  lag(College Visits, 35) & 0.350$^{*}$ & 0.638$^{***}$ & 0.729$^{***}$ & 0.791$^{***}$ \\ 
  & (0.190) & (0.193) & (0.198) & (0.190) \\ 
  lag(K-12 School Visits, 35) & 0.405$^{***}$ & 0.275 &  &  \\ 
  & (0.146) & (0.207) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 35) &  & 0.706$^{**}$ &  &  \\ 
  &  & (0.293) &  &  \\ 
  lag(Open K-12 In-person, 35) &  &  & $-$0.020 & 0.015 \\ 
  &  &  & (0.057) & (0.069) \\ 
  lag(Open K-12 Hybrid, 35) &  &  & $-$0.008 & $-$0.050$^{*}$ \\ 
  &  &  & (0.029) & (0.030) \\ 
  lag(Open K-12 Remote, 35) &  &  & $-$0.044 & $-$0.111$^{***}$ \\ 
  &  &  & (0.032) & (0.043) \\ 
  lag(full\_staff\_dum, 35) &  &  &  & 0.054 \\ 
  &  &  &  & (0.097) \\ 
  lag(hybrid\_staff\_dum, 35) &  &  &  & 0.145$^{***}$ \\ 
  &  &  &  & (0.054) \\ 
  lag(log(Deaths), 35) & $-$0.655$^{***}$ & $-$0.664$^{***}$ & $-$0.651$^{***}$ & $-$0.661$^{***}$ \\ 
  & (0.013) & (0.013) & (0.013) & (0.013) \\ 
  lag(lag(log(Deaths), 7), 35) & $-$0.046$^{***}$ & $-$0.051$^{***}$ & $-$0.044$^{***}$ & $-$0.050$^{***}$ \\ 
  & (0.006) & (0.007) & (0.007) & (0.007) \\ 
  lag(lag(log(Deaths), 14), 35) & $-$0.061$^{***}$ & $-$0.065$^{***}$ & $-$0.059$^{***}$ & $-$0.063$^{***}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
  lag(Full-time Workplace Visits, 35) & $-$1.142 & $-$1.058 & 0.965 & 0.590 \\ 
  & (0.961) & (0.967) & (1.015) & (1.015) \\ 
  lag(Part-time Workplace Visits, 35) & 2.627$^{***}$ & 1.598$^{**}$ & 2.495$^{***}$ & 2.147$^{***}$ \\ 
  & (0.686) & (0.777) & (0.722) & (0.750) \\ 
  lag(Staying Home Devices, 35) & 0.347$^{**}$ & 0.423$^{***}$ & 0.327$^{**}$ & 0.496$^{***}$ \\ 
  & (0.156) & (0.145) & (0.160) & (0.140) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 561,081 & 438,109 & 497,767 & 425,792 \\ 
R$^{2}$ & 0.274 & 0.280 & 0.279 & 0.283 \\ 
Adjusted R$^{2}$ & 0.268 & 0.274 & 0.273 & 0.276 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 28) & $-$0.044$^{***}$ & $-$0.051$^{***}$ & $-$0.053$^{***}$ & $-$0.049$^{***}$ \\ 
  & (0.010) & (0.012) & (0.013) & (0.014) \\ 
  lag(Ban gatherings, 28) & $-$0.005 & $-$0.031 & $-$0.014 & $-$0.022 \\ 
  & (0.023) & (0.029) & (0.026) & (0.030) \\ 
  lag(Stay at home, 28) & $-$0.160$^{***}$ & $-$0.144$^{***}$ & $-$0.128$^{***}$ & $-$0.102$^{***}$ \\ 
  & (0.021) & (0.021) & (0.023) & (0.023) \\ 
  lag(College Visits, 28) & 0.101$^{**}$ & 0.114$^{*}$ & 0.142$^{***}$ & 0.152$^{***}$ \\ 
  & (0.041) & (0.059) & (0.046) & (0.058) \\ 
  lag(K-12 Visits, 28) & 0.023 & $-$0.138$^{**}$ &  &  \\ 
  & (0.059) & (0.064) &  &  \\ 
  lag(K-12 Visits\_staff\_dum, 28) &  & 0.127$^{*}$ &  &  \\ 
  &  & (0.065) &  &  \\ 
  lag(Open K-12 In-person, 28) &  &  & 0.008 & 0.009 \\ 
  &  &  & (0.014) & (0.017) \\ 
  lag(Open K-12 Hybrid, 28) &  &  & 0.034$^{***}$ & 0.036$^{***}$ \\ 
  &  &  & (0.009) & (0.011) \\ 
  lag(Open K-12 Remote, 28) &  &  & 0.047$^{***}$ & 0.045$^{***}$ \\ 
  &  &  & (0.011) & (0.011) \\ 
  lag(full\_staff\_dum, 28) &  &  &  & 0.036$^{**}$ \\ 
  &  &  &  & (0.015) \\ 
  lag(hybrid\_staff\_dum, 28) &  &  &  & 0.009 \\ 
  &  &  &  & (0.016) \\ 
  lag(log(Deaths), 28d lag, 28) & $-$0.046$^{***}$ & $-$0.051$^{***}$ & $-$0.049$^{***}$ & $-$0.053$^{***}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
  lag(lag(log(Deaths), 28d lag, 7), 28) & $-$0.034$^{***}$ & $-$0.036$^{***}$ & $-$0.035$^{***}$ & $-$0.036$^{***}$ \\ 
  & (0.003) & (0.005) & (0.004) & (0.005) \\ 
  lag(lag(log(Deaths), 28d lag, 14), 28) & $-$0.021$^{***}$ & $-$0.017$^{***}$ & $-$0.019$^{***}$ & $-$0.015$^{***}$ \\ 
  & (0.004) & (0.004) & (0.004) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 628,054 & 490,561 & 557,212 & 476,787 \\ 
R$^{2}$ & 0.048 & 0.049 & 0.049 & 0.049 \\ 
Adjusted R$^{2}$ & 0.041 & 0.040 & 0.042 & 0.041 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths21-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 21) & $-$0.019$^{**}$ & $-$0.018$^{**}$ & $-$0.028$^{***}$ & $-$0.023$^{**}$ \\ 
  & (0.009) & (0.009) & (0.009) & (0.009) \\ 
  lag(Ban gatherings, 21) & $-$0.044 & $-$0.056$^{**}$ & $-$0.053$^{**}$ & $-$0.055$^{**}$ \\ 
  & (0.027) & (0.025) & (0.027) & (0.025) \\ 
  lag(Stay at home, 21) & $-$0.087$^{***}$ & $-$0.076$^{**}$ & $-$0.078$^{***}$ & $-$0.067$^{**}$ \\ 
  & (0.032) & (0.030) & (0.030) & (0.029) \\ 
  lag(College Visits, 21) & 0.142$^{***}$ & 0.181$^{***}$ & 0.189$^{***}$ & 0.170$^{***}$ \\ 
  & (0.047) & (0.057) & (0.058) & (0.055) \\ 
  lag(K-12 Visits, 21) & 0.160$^{***}$ & 0.060 &  &  \\ 
  & (0.048) & (0.066) &  &  \\ 
  lag(K-12 Visits\_staff\_dum, 21) &  & 0.174$^{**}$ &  &  \\ 
  &  & (0.073) &  &  \\ 
  lag(Open K-12 In-person, 21) &  &  & $-$0.002 & $-$0.012 \\ 
  &  &  & (0.019) & (0.019) \\ 
  lag(Open K-12 Hybrid, 21) &  &  & 0.013 & 0.014 \\ 
  &  &  & (0.014) & (0.014) \\ 
  lag(Open K-12 Remote, 21) &  &  & 0.018 & 0.015 \\ 
  &  &  & (0.015) & (0.017) \\ 
  lag(full\_staff\_dum, 21) &  &  &  & 0.050$^{***}$ \\ 
  &  &  &  & (0.016) \\ 
  lag(hybrid\_staff\_dum, 21) &  &  &  & 0.017 \\ 
  &  &  &  & (0.015) \\ 
  lag(log(Deaths), 28d lag, 21) & $-$0.053$^{***}$ & $-$0.049$^{***}$ & $-$0.052$^{***}$ & $-$0.047$^{***}$ \\ 
  & (0.004) & (0.005) & (0.004) & (0.006) \\ 
  lag(lag(log(Deaths), 28d lag, 7), 21) & $-$0.036$^{***}$ & $-$0.041$^{***}$ & $-$0.037$^{***}$ & $-$0.042$^{***}$ \\ 
  & (0.004) & (0.005) & (0.005) & (0.005) \\ 
  lag(lag(log(Deaths), 28d lag, 14), 21) & $-$0.031$^{***}$ & $-$0.032$^{***}$ & $-$0.032$^{***}$ & $-$0.033$^{***}$ \\ 
  & (0.004) & (0.005) & (0.004) & (0.005) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 628,061 & 490,568 & 557,219 & 476,794 \\ 
R$^{2}$ & 0.049 & 0.050 & 0.050 & 0.051 \\ 
Adjusted R$^{2}$ & 0.042 & 0.042 & 0.043 & 0.042 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths321-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{Death Growth Rates3} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 21) & $-$0.305$^{***}$ & $-$0.287$^{***}$ & $-$0.271$^{***}$ & $-$0.264$^{***}$ \\ 
  & (0.043) & (0.041) & (0.048) & (0.046) \\ 
  lag(Ban gatherings, 21) & $-$0.313$^{***}$ & $-$0.368$^{***}$ & $-$0.366$^{***}$ & $-$0.373$^{***}$ \\ 
  & (0.043) & (0.077) & (0.051) & (0.077) \\ 
  lag(Stay at Staying Home Devices, 21) & 0.171$^{*}$ & 0.176$^{*}$ & 0.188$^{**}$ & 0.172$^{*}$ \\ 
  & (0.092) & (0.090) & (0.091) & (0.091) \\ 
  lag(College Visits, 21) & 0.503$^{*}$ & 0.620$^{***}$ & 0.713$^{***}$ & 0.552$^{**}$ \\ 
  & (0.265) & (0.235) & (0.247) & (0.240) \\ 
  lag(K-12 School Visits, 21) & 1.627$^{***}$ & 0.774$^{**}$ &  &  \\ 
  & (0.371) & (0.376) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 21) &  & 1.572$^{***}$ &  &  \\ 
  &  & (0.373) &  &  \\ 
  lag(Open K-12 In-person, 21) &  &  & 0.051 & 0.008 \\ 
  &  &  & (0.076) & (0.098) \\ 
  lag(Open K-12 Hybrid, 21) &  &  & 0.068 & $-$0.025 \\ 
  &  &  & (0.047) & (0.040) \\ 
  lag(Open K-12 Remote, 21) &  &  & $-$0.120$^{***}$ & $-$0.212$^{***}$ \\ 
  &  &  & (0.037) & (0.050) \\ 
  lag(full\_staff\_dum, 21) &  &  &  & 0.231$^{*}$ \\ 
  &  &  &  & (0.125) \\ 
  lag(hybrid\_staff\_dum, 21) &  &  &  & 0.344$^{***}$ \\ 
  &  &  &  & (0.072) \\ 
  lag(log(Deaths), 21) & $-$0.549$^{***}$ & $-$0.527$^{***}$ & $-$0.535$^{***}$ & $-$0.520$^{***}$ \\ 
  & (0.009) & (0.009) & (0.009) & (0.009) \\ 
  lag(lag(log(Deaths), 7), 21) & $-$0.612$^{***}$ & $-$0.596$^{***}$ & $-$0.604$^{***}$ & $-$0.592$^{***}$ \\ 
  & (0.006) & (0.006) & (0.006) & (0.006) \\ 
  lag(lag(log(Deaths), 14), 21) & $-$0.661$^{***}$ & $-$0.644$^{***}$ & $-$0.656$^{***}$ & $-$0.640$^{***}$ \\ 
  & (0.006) & (0.006) & (0.006) & (0.006) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 435,781 & 341,142 & 386,863 & 331,674 \\ 
R$^{2}$ & 0.662 & 0.657 & 0.661 & 0.658 \\ 
Adjusted R$^{2}$ & 0.659 & 0.654 & 0.658 & 0.655 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths35-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{d3log(Deaths)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(Mandatory mask, 35) & $-$0.141$^{***}$ & $-$0.115$^{***}$ & $-$0.148$^{***}$ & $-$0.115$^{***}$ \\ 
  & (0.028) & (0.026) & (0.029) & (0.027) \\ 
  lag(Ban gatherings, 35) & $-$0.245$^{***}$ & $-$0.325$^{***}$ & $-$0.279$^{***}$ & $-$0.330$^{***}$ \\ 
  & (0.077) & (0.096) & (0.079) & (0.098) \\ 
  lag(Stay at Staying Home Devices, 35) & $-$0.222$^{***}$ & $-$0.153$^{**}$ & $-$0.180$^{***}$ & $-$0.141$^{**}$ \\ 
  & (0.060) & (0.065) & (0.066) & (0.071) \\ 
  lag(College Visits, 35) & 0.288 & 0.531$^{***}$ & 0.540$^{***}$ & 0.565$^{***}$ \\ 
  & (0.188) & (0.192) & (0.192) & (0.185) \\ 
  lag(K-12 School Visits, 35) & 0.729$^{***}$ & 0.393$^{**}$ &  &  \\ 
  & (0.118) & (0.184) &  &  \\ 
  lag(K-12 School Visits\_staff\_dum, 35) &  & 0.753$^{**}$ &  &  \\ 
  &  & (0.293) &  &  \\ 
  lag(Open K-12 In-person, 35) &  &  & 0.023 & 0.032 \\ 
  &  &  & (0.058) & (0.071) \\ 
  lag(Open K-12 Hybrid, 35) &  &  & 0.023 & $-$0.032 \\ 
  &  &  & (0.029) & (0.031) \\ 
  lag(Open K-12 Remote, 35) &  &  & $-$0.053 & $-$0.114$^{***}$ \\ 
  &  &  & (0.032) & (0.044) \\ 
  lag(full\_staff\_dum, 35) &  &  &  & 0.080 \\ 
  &  &  &  & (0.097) \\ 
  lag(hybrid\_staff\_dum, 35) &  &  &  & 0.157$^{***}$ \\ 
  &  &  &  & (0.053) \\ 
  lag(log(Deaths), 35) & $-$0.658$^{***}$ & $-$0.665$^{***}$ & $-$0.655$^{***}$ & $-$0.662$^{***}$ \\ 
  & (0.013) & (0.013) & (0.013) & (0.013) \\ 
  lag(lag(log(Deaths), 7), 35) & $-$0.048$^{***}$ & $-$0.051$^{***}$ & $-$0.047$^{***}$ & $-$0.050$^{***}$ \\ 
  & (0.006) & (0.007) & (0.007) & (0.007) \\ 
  lag(lag(log(Deaths), 14), 35) & $-$0.062$^{***}$ & $-$0.066$^{***}$ & $-$0.060$^{***}$ & $-$0.065$^{***}$ \\ 
  & (0.005) & (0.006) & (0.005) & (0.006) \\ 
 \hline \\[-1.8ex] 
week & Yes & Yes & Yes & Yes \\ 
state & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
Observations & 561,075 & 438,106 & 497,770 & 425,789 \\ 
R$^{2}$ & 0.274 & 0.280 & 0.279 & 0.283 \\ 
Adjusted R$^{2}$ & 0.268 & 0.274 & 0.272 & 0.276 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/summary.tex <==
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
dlogdc & 698,278 & 0.099 & 0.901 & $-$8.107 & $-$0.288 & 0.495 & 8.002 \\ 
dlogdd & 698,278 & 0.023 & 0.790 & $-$6.170 & 0.000 & 0.000 & 6.170 \\ 
dcase\_capita & 703,324 & 1.423 & 2.303 & 0.0002 & 0.196 & 1.695 & 118.235 \\ 
ddeath\_capita & 703,324 & 0.049 & 0.085 & 0.0001 & 0.011 & 0.053 & 3.109 \\ 
college & 728,228 & 0.010 & 0.031 & 0.000 & 0.000 & 0.008 & 1.827 \\ 
school & 728,228 & 0.074 & 0.072 & 0.000 & 0.024 & 0.103 & 1.167 \\ 
pschoolfull & 646,816 & 0.079 & 0.207 & 0.000 & 0.000 & 0.000 & 1.000 \\ 
pschoolhybrid & 646,816 & 0.224 & 0.357 & 0.000 & 0.000 & 0.424 & 1.000 \\ 
pschoolremote & 646,816 & 0.078 & 0.227 & 0.000 & 0.000 & 0.000 & 1.000 \\ 
staff\_dum & 577,680 & 0.293 & 0.455 & 0.000 & 0.000 & 1.000 & 1.000 \\ 
pmask & 728,944 & 0.461 & 0.495 & 0 & 0 & 1 & 1 \\ 
pgather50 & 728,944 & 0.658 & 0.472 & 0 & 0 & 1 & 1 \\ 
pshelter & 728,944 & 0.143 & 0.345 & 0 & 0 & 0 & 1 \\ 
fullwork & 728,206 & 0.054 & 0.018 & 0.010 & 0.042 & 0.061 & 0.484 \\ 
partwork & 728,206 & 0.101 & 0.025 & 0.023 & 0.084 & 0.113 & 0.567 \\ 
home & 728,206 & 0.342 & 0.116 & 0.021 & 0.267 & 0.393 & 3.657 \\ 
bar & 728,228 & 0.012 & 0.024 & 0.000 & 0.0001 & 0.015 & 1.461 \\ 
restaurant & 728,228 & 0.250 & 0.175 & 0.000 & 0.150 & 0.315 & 4.261 \\ 
gym & 728,228 & 0.017 & 0.022 & 0.000 & 0.000 & 0.026 & 0.786 \\ 
church & 728,228 & 0.025 & 0.018 & 0.000 & 0.014 & 0.032 & 0.583 \\ 
dlogtests & 698,278 & 0.067 & 0.932 & $-$13.616 & $-$0.050 & 0.175 & 13.111 \\ 
pop & 706,966 & 0.104 & 0.331 & 0.0002 & 0.012 & 0.071 & 10.106 \\ 
\hline \\[-1.8ex] 
\end{tabular} 

==> tables_and_figures/summary_fullbefore.tex <==
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
dlogdc & 52,258 & 0.091 & 1.055 & $-$4.970 & $-$0.405 & 0.693 & 6.094 \\ 
dlogdd & 52,258 & 0.013 & 0.510 & $-$3.890 & 0.000 & 0.000 & 3.890 \\ 
logdc & 54,995 & 1.072 & 1.854 & $-$1.000 & $-$1.000 & 2.303 & 9.256 \\ 
logdd & 54,995 & $-$0.756 & 0.729 & $-$1.000 & $-$1.000 & $-$1.000 & 5.257 \\ 
college & 67,070 & 0.005 & 0.019 & 0.000 & 0.000 & 0.003 & 0.599 \\ 
school & 67,070 & 0.045 & 0.038 & 0.000 & 0.021 & 0.057 & 0.715 \\ 
pschoolfull & 67,107 & 0.000 & 0.000 & 0 & 0 & 0 & 0 \\ 
pschoolhybrid & 67,107 & 0.003 & 0.027 & 0 & 0 & 0 & 0 \\ 
pschoolremote & 67,107 & 0.001 & 0.011 & 0 & 0 & 0 & 0 \\ 
staff\_dum & 62,099 & 0.477 & 0.499 & 0.000 & 0.000 & 1.000 & 1.000 \\ 
pmask & 67,107 & 0.172 & 0.372 & 0 & 0 & 0 & 1 \\ 
pgather50 & 67,107 & 0.564 & 0.489 & 0.000 & 0.000 & 1.000 & 1.000 \\ 
pshelter & 67,107 & 0.172 & 0.367 & 0 & 0 & 0 & 1 \\ 
fullwork & 67,070 & 0.047 & 0.015 & 0.010 & 0.039 & 0.051 & 0.257 \\ 
partwork & 67,070 & 0.098 & 0.021 & 0.033 & 0.085 & 0.109 & 0.278 \\ 
home & 67,070 & 0.374 & 0.143 & 0.048 & 0.289 & 0.422 & 2.892 \\ 
bar & 67,070 & 0.012 & 0.026 & 0.000 & 0.000 & 0.015 & 1.461 \\ 
restaurant & 67,070 & 0.185 & 0.147 & 0.000 & 0.089 & 0.248 & 2.420 \\ 
gym & 67,070 & 0.010 & 0.018 & 0.000 & 0.000 & 0.014 & 0.662 \\ 
church & 67,070 & 0.028 & 0.022 & 0.000 & 0.014 & 0.036 & 0.287 \\ 
dlogtests & 52,240 & 0.089 & 1.416 & $-$12.945 & $-$0.057 & 0.205 & 13.105 \\ 
pop & 57,150 & 0.038 & 0.147 & 0.001 & 0.006 & 0.025 & 1.951 \\ 
\hline \\[-1.8ex] 
\end{tabular} 

==> tables_and_figures/summary_plan.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\
  & Case  & Death  & Cases & Deaths & K-12 Sch. & Workplace   & Restaurant  \\
  &  Growth &  Growth & per 1000 & per 1000 &  Visits &  Visits & Visits \\ \hline
 In-person \\
 \qquad Before Opening \\
\qquad\quad Mean & 0.091 & 0.013 & 0.57 & 0.06 & 0.045 & 0.047 & 0.19 \\
   & (0.011) & (0.0027) & (0.031) & (0.003) & (0.0017) & (0.00061) & (0.0069) \\
 \qquad\quad N & 52258 & 52258 & 54995 & 54995 & 67070 & 67070 & 67070 \\
\qquad After Opening \\
\qquad\quad Mean & 0.14 & 0.034 & 3 & 0.1 & 0.16 & 0.073 & 0.19 \\
   & (0.014) & (0.0063) & (0.2) & (0.0052) & (0.0049) & (0.0011) & (0.0061) \\
 \qquad\quad N & 45749 & 45749 & 45827 & 45827 & 46030 & 46030 & 46030 \\
\qquad Difference \\
\qquad\quad Mean & 0.052 & 0.021 & 2.5 & 0.044 & 0.12 & 0.026 & 0.003 \\
   & (0.018) & (0.0072) & (0.2) & (0.0041) & (0.0044) & (0.00098) & (0.0038) \\
 Hybrid \\
 \qquad Before Opening \\
\qquad\quad Mean & 0.096 & 0.024 & 0.66 & 0.035 & 0.036 & 0.045 & 0.24 \\
   & (0.012) & (0.0056) & (0.031) & (0.001) & (0.0012) & (0.00036) & (0.0054) \\
 \qquad\quad N & 234820 & 234820 & 243321 & 243321 & 260573 & 260551 & 260573 \\
\qquad After Opening \\
\qquad\quad Mean & 0.12 & 0.042 & 2.4 & 0.057 & 0.13 & 0.064 & 0.25 \\
   & (0.012) & (0.0063) & (0.13) & (0.002) & (0.0028) & (0.00064) & (0.0039) \\
 \qquad\quad N & 166605 & 166605 & 166660 & 166660 & 167206 & 167206 & 167206 \\
\qquad Difference \\
\qquad\quad Mean & 0.025 & 0.019 & 1.7 & 0.022 & 0.09 & 0.019 & 0.0068 \\
   & (0.016) & (0.0083) & (0.14) & (0.0018) & (0.0028) & (0.00063) & (0.0043) \\
 Remote \\
 \qquad Before Opening \\
\qquad\quad Mean & 0.099 & 0.035 & 0.74 & 0.032 & 0.032 & 0.045 & 0.28 \\
   & (0.012) & (0.0078) & (0.035) & (0.0017) & (0.0012) & (0.00043) & (0.0085) \\
 \qquad\quad N & 76796 & 76796 & 78581 & 78581 & 82165 & 82165 & 82165 \\
\qquad After Opening \\
\qquad\quad Mean & 0.1 & 0.033 & 1.9 & 0.047 & 0.088 & 0.058 & 0.29 \\
   & (0.012) & (0.0091) & (0.11) & (0.0029) & (0.0034) & (0.00073) & (0.0075) \\
 \qquad\quad N & 50127 & 50127 & 50048 & 50048 & 50183 & 50183 & 50183 \\
\qquad Difference \\
\qquad\quad Mean & 0.0044 & -0.0024 & 1.2 & 0.015 & 0.056 & 0.013 & 0.0086 \\
   & (0.017) & (0.012) & (0.12) & (0.0023) & (0.003) & (0.00063) & (0.0057) \\

  \hline \\[-1.8ex]
\end{tabular}


==> tables_and_figures/summary_plan2.tex <==
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
  & Case  & Death  & Cases & Deaths & K-12 School & Workplace   & Restaurant  \\
Statistic &  Growth &  Growth & per 1000 & per 1000 &  Visits &  Visits & Visits \\
In-person before Opening&&&&&&&\\
Mean & 0.091 & 0.012 & 0.624 & 0.062 & 0.055 & 0.049 & 0.186 \\ 
St. Dev. & 1.055 & 0.518 & 1.209 & 0.080 & 0.056 & 0.016 & 0.147 \\ 
N & 58,549 & 58,549 & 61,324 & 61,324 & 73,486 & 73,486 & 73,486 \\ 
In-person after Opening&&&&&&&\\
Mean & 0.151 & 0.039 & 3.350 & 0.108 & 0.161 & 0.074 & 0.186 \\ 
St. Dev. & 0.879 & 0.751 & 3.784 & 0.152 & 0.100 & 0.022 & 0.129 \\ 
N & 39,458 & 39,458 & 39,498 & 39,498 & 39,614 & 39,614 & 39,614 \\ 
Hybrid before Opening&&&&&&&\\
Mean & 0.090 & 0.022 & 0.705 & 0.036 & 0.044 & 0.047 & 0.244 \\ 
St. Dev. & 0.985 & 0.737 & 1.454 & 0.057 & 0.044 & 0.015 & 0.175 \\ 
N & 259,037 & 259,037 & 267,544 & 267,544 & 284,907 & 284,885 & 284,907 \\ 
Hybrid after Opening&&&&&&&\\
Mean & 0.135 & 0.048 & 2.580 & 0.059 & 0.127 & 0.065 & 0.247 \\ 
St. Dev. & 0.766 & 0.912 & 2.778 & 0.099 & 0.076 & 0.019 & 0.156 \\ 
N & 142,388 & 142,388 & 142,437 & 142,437 & 142,872 & 142,872 & 142,872 \\ 
Remote before Opening&&&&&&&\\
Mean & 0.091 & 0.033 & 0.777 & 0.033 & 0.036 & 0.046 & 0.280 \\ 
St. Dev. & 0.876 & 0.830 & 1.166 & 0.058 & 0.037 & 0.011 & 0.188 \\ 
N & 84,302 & 84,302 & 86,073 & 86,073 & 89,685 & 89,685 & 89,685 \\ 
Remote after Opening&&&&&&&\\
N & 42,621 & 42,621 & 42,556 & 42,556 & 42,663 & 42,663 & 42,663 \\ 
Mean & 0.121 & 0.036 & 2.083 & 0.048 & 0.089 & 0.059 & 0.285 \\ 
St. Dev. & 0.662 & 0.955 & 2.311 & 0.086 & 0.075 & 0.016 & 0.174 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 
